Is the diurnal pattern sufficient to explain intraday variation in volatility? A nonparametric assessment

In this paper, we propose a nonparametric way to test the hypothesis that time-variation in intraday volatility is caused solely by a deterministic and recurrent diurnal pattern. We assume that noisy high-frequency data from a discretely sampled jump-diffusion process are available. The test is then based on asset returns, which are deflated by the seasonal component and therefore homoskedastic under the null. To construct our test statistic, we extend the concept of pre-averaged bipower variation to a general It\^o semimartingale setting via a truncation device. We prove a central limit theorem for this statistic and construct a positive semi-definite estimator of the asymptotic covariance matrix. The $t$-statistic (after pre-averaging and jump-truncation) diverges in the presence of stochastic volatility and has a standard normal distribution otherwise. We show that replacing the true diurnal factor with a model-free jump- and noise-robust estimator does not affect the asymptotic theory. A Monte Carlo simulation also shows this substitution has no discernable impact in finite samples. The test is, however, distorted by small infinite-activity price jumps. To improve inference, we propose a new bootstrap approach, which leads to almost correctly sized tests of the null hypothesis. We apply the developed framework to a large cross-section of equity high-frequency data and find that the diurnal pattern accounts for a rather significant fraction of intraday variation in volatility, but important sources of heteroskedasticity remain present in the data.

==> tables/sim-theta=0.333-beta=-0.5-i.tex <==
\begin{sidewaystable}[p!]
\setlength{ \tabcolsep}{0.09cm}
\begin{center}
\caption{Infeasible rejection rate at 5\% level of significance with $\theta = 0.333$ and $\varphi = -0.5$.
\label{table:sim-theta=0.333-beta=-0.5-i.tex}}
\vspace*{-0.25cm}
\begin{small}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\hline \hline
& & & \multicolumn{15}{c}{$\mathcal{H}_{0}$ : deterministic volatility} & & \multicolumn{15}{c}{$\mathcal{H}_{a}$ : stochastic volatility}\\ \cline{4-18} \cline{20-34}
& & & \multicolumn{7}{c}{size} & & \multicolumn{7}{c}{avg. block length} & & \multicolumn{7}{c}{power} & & \multicolumn{7}{c}{avg. block length}\\ \cline{4-10} \cline{12-18} \cline{20-26} \cline{28-34}
& & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$\\
\multicolumn{10}{l}{Panel A: $\xi^{2} = 0.0001$}\\
$n = $& 390 && 23.0 && 6.1 & 6.3 && 9.3 & 9.9&& 136&& 130&  131&& 132&  131 && 63.1 && 33.5 & 33.9 && 40.0 & 40.3&& 136&& 131&  130&& 132&  132\\
& 780 && 17.1 && 5.1 & 4.4 && 7.6 & 7.9&& 216&& 210&  211&& 210&  211 && 63.3 && 42.2 & 41.3 && 45.5 & 44.8&& 216&& 211&  212&& 211&  210\\
& 1560 && 12.1 && 4.4 & 4.5 && 5.5 & 5.7&& 343&& 335&  336&& 336&  333 && 65.6 && 47.4 & 48.3 && 50.5 & 49.7&& 341&& 335&  334&& 335&  336\\
& 4680 && 10.7 && 5.0 & 4.9 && 5.7 & 6.3&& 708&& 701&  700&& 697&  695 && 70.3 && 59.4 & 59.0 && 60.2 & 60.1&& 706&& 698&  700&& 697&  698\\
& 7800 && 10.2 && 6.0 & 5.4 && 7.2 & 7.5&& 998&& 981&  986&& 982&  985 && 74.3 && 66.2 & 65.9 && 66.6 & 65.7&& 995&& 977&  980&& 983&  978\\
& 11700 && 10.2 && 5.6 & 5.7 && 6.8 & 7.2&& 1,302&& 1,292&  1,291&& 1,297&  1,286 && 78.5 && 70.5 & 71.4 && 70.2 & 70.5&& 1,305&& 1,289&  1,286&& 1,288&  1,278\\
& 23400 && 8.1 && 5.1 & 5.5 && 5.9 & 5.9&& 2,068&& 2,042&  2,046&& 2,040&  2,046 && 83.2 && 78.7 & 79.3 && 79.7 & 79.7&& 2,067&& 2,045&  2,045&& 2,045&  2,038\\
\\
\multicolumn{10}{l}{Panel B: $\xi^{2} = 0.0010$}\\
$n = $& 390 && 23.7 && 5.7 & 6.9 && 9.4 & 9.7&& 136&& 131&  131&& 132&  131 && 60.6 && 32.0 & 31.6 && 38.4 & 39.1&& 136&& 131&  131&& 131&  131\\
& 780 && 16.9 && 5.0 & 4.9 && 6.9 & 7.2&& 214&& 211&  210&& 211&  210 && 62.7 && 40.5 & 39.8 && 44.3 & 44.2&& 216&& 211&  211&& 210&  211\\
& 1560 && 13.4 && 4.3 & 4.0 && 5.8 & 5.7&& 342&& 335&  336&& 338&  337 && 63.2 && 47.2 & 46.0 && 49.9 & 49.7&& 340&& 335&  336&& 334&  336\\
& 4680 && 10.9 && 4.8 & 5.2 && 6.6 & 6.6&& 706&& 698&  701&& 697&  699 && 69.5 && 60.3 & 60.1 && 60.2 & 59.6&& 706&& 696&  700&& 694&  700\\
& 7800 && 9.7 && 5.1 & 5.5 && 6.4 & 6.2&& 998&& 980&  988&& 977&  982 && 72.3 && 64.6 & 64.5 && 64.5 & 64.4&& 998&& 982&  986&& 982&  986\\
& 11700 && 10.1 && 5.7 & 5.5 && 6.7 & 7.3&& 1,308&& 1,294&  1,287&& 1,287&  1,286 && 76.9 && 69.8 & 70.7 && 69.6 & 69.8&& 1,306&& 1,284&  1,294&& 1,285&  1,294\\
& 23400 && 8.3 && 5.7 & 5.5 && 6.0 & 5.8&& 2,062&& 2,043&  2,051&& 2,053&  2,050 && 83.0 && 78.5 & 78.5 && 78.6 & 79.0&& 2,054&& 2,053&  2,051&& 2,052&  2,048\\
\\
\multicolumn{10}{l}{Panel C: $\xi^{2} = 0.0100$}\\
$n = $& 390 && 24.7 && 7.3 & 7.8 && 11.3 & 10.9&& 136&& 131&  131&& 131&  131 && 48.2 && 21.9 & 21.1 && 25.5 & 26.0&& 135&& 131&  131&& 130&  131\\
& 780 && 16.2 && 3.7 & 4.0 && 6.5 & 7.0&& 215&& 211&  211&& 212&  211 && 52.1 && 24.6 & 24.2 && 29.8 & 30.2&& 217&& 210&  211&& 210&  210\\
& 1560 && 14.7 && 5.2 & 5.2 && 8.0 & 7.9&& 341&& 336&  334&& 336&  335 && 49.4 && 30.8 & 31.3 && 35.2 & 35.8&& 340&& 336&  335&& 335&  337\\
& 4680 && 12.0 && 6.2 & 6.1 && 7.5 & 7.7&& 706&& 705&  698&& 698&  701 && 60.9 && 47.5 & 48.0 && 49.0 & 49.0&& 707&& 703&  703&& 700&  700\\
& 7800 && 10.1 && 4.0 & 4.2 && 5.9 & 6.2&& 998&& 980&  991&& 982&  987 && 65.1 && 54.9 & 55.0 && 55.1 & 55.0&& 997&& 978&  979&& 980&  973\\
& 11700 && 9.0 && 5.7 & 5.4 && 5.9 & 6.1&& 1,298&& 1,287&  1,295&& 1,291&  1,296 && 68.0 && 60.2 & 59.5 && 60.5 & 60.0&& 1,294&& 1,290&  1,291&& 1,282&  1,290\\
& 23400 && 8.9 && 5.7 & 6.1 && 7.3 & 6.8&& 2,055&& 2,050&  2,036&& 2,045&  2,039 && 73.7 && 68.3 & 68.1 && 68.7 & 68.3&& 2,060&& 2,045&  2,041&& 2,052&  2,037\\
\hline \hline
\end{tabular}
\end{small}\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate from a model with drift, volatility, infinite-activity jumps and microstructure noise. We test the hypothesis that $\sigma_{t} = \sigma \sigma_{u,t}$ is a deterministic function of time (induced by diurnal variation) and report rejection rates both under $\mathcal{H}_{0}$ (size) and $\mathcal{H}_{a}$ (power). In the latter, $\sigma_{t}  = \sigma_{sv,t} \sigma_{u,t}$ is also time-varying due to a two-factor SV structure. $\theta$ is a tuning parameter that is used to compute the pre-averaging window $k_{n} = [\theta \sqrt{n}]$, $\varphi$ is the MA(1) coefficient in the noise process, $n$ is the sample size, and $\xi^{2}$ controls the magnitude of noise relative to volatility. CLT is for the asymptotic theory from \eqref{equation:clt}, while $z_{\text{wb}\cdot}$ and $t_{\text{wb}\cdot}$ are rejection rates based on the percentile and percentile-$t$ bootstrap test for two choices of the external random variable $u$. We made 1,000 Monte Carlo trials with 999 bootstrap replica in each simulation. Further details can be found in Section \ref{section:montecarlo}.} 
\end{scriptsize}
\end{center}
\end{sidewaystable}

==> tables/sim-theta=1.000-beta=-0.5-i.tex <==
\begin{sidewaystable}[p!]
\setlength{ \tabcolsep}{0.09cm}
\begin{center}
\caption{Infeasible rejection rate at 5\% level of significance with $\theta = 1.000$ and $\varphi = -0.5$.
\label{table:sim-theta=1.000-beta=-0.5-i.tex}}
\vspace*{-0.25cm}
\begin{small}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\hline \hline
& & & \multicolumn{15}{c}{$\mathcal{H}_{0}$ : deterministic volatility} & & \multicolumn{15}{c}{$\mathcal{H}_{a}$ : stochastic volatility}\\ \cline{4-18} \cline{20-34}
& & & \multicolumn{7}{c}{size} & & \multicolumn{7}{c}{avg. block length} & & \multicolumn{7}{c}{power} & & \multicolumn{7}{c}{avg. block length}\\ \cline{4-10} \cline{12-18} \cline{20-26} \cline{28-34}
& & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$
  & & CLT & &  $z_{ \text{wb1}}$ & $z_{ \text{wb2}}$ && $t_{ \text{wb1}}$ & $t_{ \text{wb2}}$\\
\multicolumn{10}{l}{Panel A: $\xi^{2} = 0.0001$}\\
$n = $& 390 && 21.1 && 9.0 & 9.1 && 11.4 & 10.9&& 135&& 130&  130&& 130&  130 && 48.3 && 24.7 & 23.6 && 28.8 & 28.9&& 135&& 131&  131&& 131&  129\\
& 780 && 13.7 && 6.0 & 5.3 && 7.1 & 7.2&& 215&& 211&  210&& 210&  210 && 43.4 && 24.2 & 23.5 && 27.7 & 27.4&& 217&& 210&  211&& 210&  211\\
& 1560 && 13.3 && 6.6 & 5.7 && 7.7 & 8.1&& 339&& 336&  336&& 336&  334 && 47.8 && 34.3 & 33.7 && 36.7 & 36.1&& 342&& 335&  335&& 336&  334\\
& 4680 && 10.7 && 6.8 & 5.5 && 7.7 & 7.2&& 708&& 702&  698&& 698&  697 && 51.8 && 43.2 & 43.5 && 43.2 & 43.4&& 708&& 695&  697&& 697&  698\\
& 7800 && 9.1 && 5.2 & 5.1 && 6.1 & 6.2&& 996&& 982&  982&& 974&  985 && 58.4 && 48.7 & 48.1 && 49.0 & 49.0&& 994&& 985&  979&& 982&  977\\
& 11700 && 9.4 && 5.3 & 5.4 && 7.0 & 6.4&& 1,296&& 1,294&  1,286&& 1,285&  1,289 && 62.6 && 53.3 & 54.2 && 53.0 & 53.2&& 1,304&& 1,293&  1,286&& 1,289&  1,284\\
& 23400 && 9.1 && 6.8 & 6.7 && 7.1 & 7.2&& 2,060&& 2,052&  2,036&& 2,059&  2,040 && 67.5 && 62.3 & 61.0 && 60.8 & 61.5&& 2,069&& 2,033&  2,036&& 2,043&  2,048\\
\\
\multicolumn{10}{l}{Panel B: $\xi^{2} = 0.0010$}\\
$n = $& 390 && 21.2 && 9.6 & 8.6 && 10.8 & 11.3&& 135&& 130&  131&& 131&  130 && 49.3 && 24.3 & 23.5 && 28.6 & 28.1&& 135&& 130&  131&& 131&  130\\
& 780 && 13.9 && 5.9 & 5.6 && 7.4 & 7.6&& 216&& 209&  211&& 210&  211 && 43.8 && 24.2 & 23.1 && 27.3 & 28.3&& 216&& 211&  211&& 211&  210\\
& 1560 && 13.3 && 6.4 & 6.1 && 7.8 & 7.9&& 339&& 335&  336&& 334&  334 && 48.0 && 34.1 & 33.3 && 36.3 & 35.9&& 340&& 336&  335&& 336&  334\\
& 4680 && 10.8 && 6.5 & 5.8 && 7.4 & 7.3&& 710&& 699&  705&& 696&  702 && 52.4 && 43.2 & 43.8 && 43.5 & 43.2&& 705&& 700&  702&& 700&  699\\
& 7800 && 9.2 && 5.2 & 5.1 && 5.8 & 5.9&& 996&& 981&  988&& 982&  981 && 58.3 && 48.2 & 48.1 && 47.8 & 48.1&& 1,000&& 981&  982&& 979&  981\\
& 11700 && 9.4 && 5.3 & 5.3 && 7.0 & 6.4&& 1,295&& 1,293&  1,285&& 1,292&  1,283 && 62.4 && 53.4 & 53.3 && 53.7 & 52.9&& 1,297&& 1,289&  1,285&& 1,278&  1,287\\
& 23400 && 9.1 && 6.5 & 6.4 && 7.4 & 7.3&& 2,047&& 2,046&  2,026&& 2,049&  2,043 && 67.3 && 61.7 & 62.1 && 60.6 & 61.1&& 2,074&& 2,045&  2,043&& 2,041&  2,052\\
\\
\multicolumn{10}{l}{Panel C: $\xi^{2} = 0.0100$}\\
$n = $& 390 && 21.6 && 9.1 & 9.0 && 12.9 & 12.2&& 135&& 131&  131&& 131&  131 && 48.9 && 24.5 & 24.2 && 28.6 & 28.0&& 136&& 131&  130&& 131&  130\\
& 780 && 14.1 && 5.6 & 5.9 && 7.5 & 8.1&& 215&& 210&  210&& 210&  210 && 42.2 && 24.0 & 23.9 && 28.0 & 27.4&& 215&& 210&  210&& 210&  210\\
& 1560 && 14.3 && 7.3 & 6.6 && 8.5 & 8.4&& 342&& 335&  336&& 336&  336 && 47.2 && 33.1 & 33.0 && 34.9 & 35.4&& 341&& 335&  334&& 337&  334\\
& 4680 && 10.2 && 5.5 & 5.6 && 7.2 & 7.3&& 707&& 701&  703&& 700&  701 && 52.3 && 41.2 & 41.0 && 42.3 & 41.8&& 708&& 700&  701&& 695&  698\\
& 7800 && 9.4 && 4.9 & 5.1 && 7.1 & 6.7&& 998&& 981&  986&& 979&  986 && 56.9 && 45.3 & 45.2 && 46.1 & 46.0&& 994&& 976&  984&& 975&  980\\
& 11700 && 9.1 && 6.0 & 5.9 && 6.8 & 6.7&& 1,298&& 1,289&  1,285&& 1,287&  1,288 && 61.1 && 51.5 & 52.0 && 51.4 & 51.1&& 1,299&& 1,284&  1,283&& 1,285&  1,290\\
& 23400 && 9.3 && 7.1 & 6.9 && 7.7 & 7.7&& 2,056&& 2,047&  2,044&& 2,044&  2,050 && 65.9 && 60.1 & 60.1 && 59.9 & 59.9&& 2,065&& 2,037&  2,044&& 2,039&  2,045\\
\hline \hline
\end{tabular}
\end{small}\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate from a model with drift, volatility, infinite-activity jumps and microstructure noise. We test the hypothesis that $\sigma_{t} = \sigma \sigma_{u,t}$ is a deterministic function of time (induced by diurnal variation) and report rejection rates both under $\mathcal{H}_{0}$ (size) and $\mathcal{H}_{a}$ (power). In the latter, $\sigma_{t}  = \sigma_{sv,t} \sigma_{u,t}$ is also time-varying due to a two-factor SV structure. $\theta$ is a tuning parameter that is used to compute the pre-averaging window $k_{n} = [\theta \sqrt{n}]$, $\varphi$ is the MA(1) coefficient in the noise process, $n$ is the sample size, and $\xi^{2}$ controls the magnitude of noise relative to volatility. CLT is for the asymptotic theory from \eqref{equation:clt}, while $z_{\text{wb}\cdot}$ and $t_{\text{wb}\cdot}$ are rejection rates based on the percentile and percentile-$t$ bootstrap test for two choices of the external random variable $u$. We made 1,000 Monte Carlo trials with 999 bootstrap replica in each simulation. Further details can be found in Section \ref{section:montecarlo}.} 
\end{scriptsize}
\end{center}
\end{sidewaystable}
